Sharp Oracle Inequalities for Low-complexity Priors

In this paper,we consider a high-dimensional statistical estimation problem in which the the number of parameters is comparable or larger than the sample size. We present a unified analysis of the performance guarantees of exponential weighted aggregation and penalized estimators with a general class of data losses and priors which encourage objects which conform to some notion of simplicity/complexity. More precisely, we show that these two estimators satisfy sharp oracle inequalities for prediction ensuring their good theoretical performances. We also highlight the differences between them. When the noise is random, we provide oracle inequalities in probability using concentration inequalities. These results are then applied to several instances including the Lasso, the group Lasso, their analysis-type counterparts, the $\ell_\infty$ and the nuclear norm penalties. All our estimators can be efficiently implemented using proximal splitting algorithms.

==> sections/conclu.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion} \label{sec:conclu}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> sections/gauges.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Low-complexity penalties} \label{sec:ewae}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The EWA estimator in \eqref{eq:EWAaggregate}-\eqref{eq:EWAaggregator} requires two essential ingredients: the data fidelity term $F$ and the prior penalty $J$. We here specify the class of such functions covered in our work, and provide illustrating examples. 

\subsection{Choice of the data loss} \label{subsec:fid}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The class of loss functions $F$ that we consider obey the following assumption:
\begin{enumerate}[label=\textbf{(H.\arabic*)},ref=\bf{(H.\arabic*)}]
\item $F(\bsu,\yy)=\varphi(\bsu) - \dotp{\bsu}{\yy}$, where $\varphi \in C^1(\RR^n)$ is strongly convex with modulus $\sigm > 0$.
%and $\nabla \varphi$ is $\sigM$-Lipschitz continuous, $\sigm > 0$ and $\sigM > 0$.
%\item For any $\yy \in \RR^n$, $F(\cdot,\yy) \in C^1(\RR^n)$ is $\sigm$-strongly convex and $\nabla F(\cdot,\yy)$ is $\sigM$-Lipschitz continuous, $\sigm > 0$ and $\sigM > 0$.
\label{assump:F}
%\item $F(\yy,\yy)=0$ and $\nabla F(\yy,\yy)=0$.
%\label{assump:gradF}
\end{enumerate}
This is reminiscent of the negative log-likelihood in the regular exponential family.
%The last assumption is very natural for a data fidelity term. Observe that the hypothesis that $F(y,y)=0$ does not entail any loss of generality and can be replaced by any constant. This is a fairly general class of loss functions.

\todo{Check if we can refine this assumption}.

\todo{Give examples}.

The following simple lemma gives useful bounds of the Bregman distance associated to $F$
\begin{lemma}
\label{lem:Fbounds}
For $F$ satisfying \ref{assump:F}, the following bounds hold
\[
\breg{F(\cdot,\yy)}{}{\bsv}{\bsu} \geq \tfrac{\sigm}{2} \norm{\bsv-\bsu}{2}^2 .
\]
If $\nabla \varphi$ is $\sigM$-Lipschitz continuous, $\sigM > 0$, then  
\[
\breg{F(\cdot,\yy)}{}{\bsv}{\bsu} \leq \tfrac{\sigM}{2} \norm{\bsv-\bsu}{2}^2 .
\]
\end{lemma}

\begin{proof}
It is immediate to see that
\[
\breg{F(\cdot,\yy)}{}{\bsv}{\bsu} =  \breg{\varphi}{}{\bsv}{\bsu}.
\]
The lower-bound is then by definition of strong convexity of $\varphi$. The upper-bound is known as the descent lemma applied to $\varphi$, see e.g. \cite[Theorem~2.1.5]{NesterovBook98}.
\end{proof}



\subsection{Choice of the prior penalty} \label{subsec:prior}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Before stating our main assumption on $J$, we start by collecting some ingredients from convex analysis that are essential to our exposition.

\paragraph{Support function}
The \emph{support function} of $\calC \subset \RR^p$ is
\[
	\sigma_{\calC}(\bsom)=\sup_{\xx \in \calC} \dotp{\bsom}{\xx} .
\]
We recall the following properties whose proofs can be found in e.g.~\cite{rockafellar1996convex,hiriart1996convex}.
\begin{lemma}
\label{lem:suppcompact}
Let $\calC$ be a non-empty set. 
\begin{enumerate}[label=(\roman*)] 
\item $\sigma_\calC$ is proper lsc and sublinear.
\item $\sigma_\calC$ is finite-valued if and only if $\calC$ is bounded.
\item If $0 \in \calC$, then $\sigma_\calC$ is non-negative. 
\item If $\calC$ is convex and compact with $0 \in \interop(\calC)$, then $\sigma_\calC$ is finite-valued and coercive.
\end{enumerate}
\end{lemma}


\paragraph{Gauges and polars}
Let $\calC \subseteq \RR^p$ be a non-empty closed convex set containing the origin.
The \emph{gauge} of $\calC$ is the function $\gauge_\calC$ defined on $\RR^p$ by
\begin{equation*}
  \gauge_\calC(\xx) =
  \inf \enscond{\lambda \geq 0}{\xx \in \lambda \calC} .
\end{equation*}

Lemma~\ref{lem:convex-gauge} hereafter recaps the main properties of a gauge that we need (see \cite{rockafellar1996convex,hiriart1996convex,vaiterimaiai13} for proofs). In particular, (ii) is a fundamental result of convex analysis that states that there is a one-to-one correspondence between gauge functions and closed convex sets containing the origin. This allows to identify sets from their gauges, and vice versa.
\begin{lemma}\label{lem:convex-gauge}
{~\\}\vspace*{-0.5cm}
\begin{enumerate}[label=(\roman*)]
\item $\gauge_\calC$ is a non-negative, lsc and sublinear function.
\item $\calC$ is the unique closed convex set containing the origin such that
\[
\calC = \enscond{\xx \in \RR^p}{\gamma_\calC(\xx) \leq 1} .
\]
\item $\gamma_\calC$ is finite-valued if, and only if, $0 \in \interop(\calC)$, in which case $\gamma_\calC$ is locally Lipschitz continuous.
\item $\gamma_\calC$ is finite-valued and coercive if, and only if, $\calC$ is compact and $0 \in \interop(\calC)$.
\end{enumerate}
\end{lemma}

Observe that $\gamma_\calC$ is a norm, having $\calC$ as its unit ball, if and only if $\calC$ is bounded with nonempty interior and symmetric.
 
We now define the polar gauge.
\begin{definition}[Polar Gauge]\label{defn:polar-gauge}
The polar of a gauge $\gamma_\calC$ is the function $\gamma_\calC^\circ$ defined by
\[
	\gamma_\calC^\circ(\bsom) = \inf\enscond{\mu \geq 0}{\dotp{\xx}{\bsom} \leq \mu \gamma_\calC(\xx), \forall \xx} .
\] 
\end{definition}
An immediate consequence is that gauges polar to each other have the property
\begin{equation}\label{eq:dualineq}
    \dotp{\xx}{\bsu} \leq \gauge_\calC(\xx) \gauge_\calC^\circ(\bsu) \quad \forall (\xx,\bsu) \in \dom(\gauge_\calC) \times \dom(\gauge_\calC^\circ) ,
\end{equation}
just as dual norms satisfy a duality inequality. In fact, polar pairs of gauges correspond to the best inequalities of this type.

\begin{lemma}\label{lem:convex-polar-gauge}
  Let $\calC \subseteq \RR^p$ be a closed convex set containing the origin.
  Then,
  \begin{enumerate}[label=(\roman*),start=2]
  \item $\gauge_\calC^\circ$ is a gauge function and $\gamma_\calC^{\circ\circ}=\gamma_\calC$.
  \item $\gamma_\calC^\circ=\gamma_{\calC^\circ}$, or equivalently
  \[
  \calC^\circ = \enscond{\xx \in \RR^p}{\gamma_\calC^\circ(\xx) \leq 1} .
  \]
\item The gauge of $\calC$ and the support function of $\calC$ are mutually polar, i.e.
  \begin{equation*}
    \gauge_\calC = \sigma_{\calC^\circ} \qandq \gauge_{\calC^\circ} = \sigma_\calC ~.
  \end{equation*}
\end{enumerate}
\end{lemma}
See \cite{rockafellar1996convex,hiriart1996convex,vaiterimaiai13} for proofs.

We are now ready to state our main assumption on $J$.
\begin{enumerate}[label=\textbf{(H.\arabic*)},ref=\bf{(H.\arabic*)},start=2]
\item $J: \RR^p \to \RR$ is the gauge of a non-empty convex compact set containing the origin as an interior point.
\label{assump:J}
\end{enumerate}
By Lemma~\ref{lem:convex-gauge}, this assumption is equivalent to saying that $J \eqdef \gamma_{\calC}$ is proper, convex, positively homogeneous, finite-valued and coercive. In turn, $J$ is locally Lipschitz continuous on $\RR^p$. Observe also that by virtue of Lemma~\ref{lem:convex-polar-gauge} and Lemma~\ref{lem:suppcompact}, the polar gauge $J^\circ \eqdef \gamma_{\calC^\circ}$ enjoys the same properties as $J$ in \ref{assump:J}.


\subsection{Decomposability of the prior penalty}\label{subsec:decomp}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We are now in position to provide an important characterization of the subdifferential mapping of a function $J$ satisfying \ref{assump:J}. This characterization will play a pivotal role in our proof of the oracle inequality. 

We start by defining some essential geometrical objects that were introduced in \cite{vaiterimaiai13,vaiterbookchap15,vaiteraism16}.
\begin{definition}[Model Subspace]\label{defn:linmod}
  Let $\xx \in \RR^p$. We denote by $\e{\xx}$ as
  \begin{equation*}
    \e{\xx} = \proj_{\Aff(\partial J(\xx))}(0).
  \end{equation*}
  We denote 
  \begin{equation*}
    \S_{\xx} = \Lin (\partial \J(\xx)) \qandq \T_{\xx} = \S_{\xx}^\bot .
  \end{equation*}
  $\T_{\xx}$ is coined the \emph{model subspace} of $\xx$ associated to $J$.
\end{definition}
When $J$ is differentiable at $\xx$, we have $\e{\xx}=\nabla J(\xx)$ and $\T_{\xx}=\RR^p$. When $J$ is the $\ell_1$-norm (Lasso), the vector $\e{\xx}$ is nothing but the sign of $\xx$. Thus, $\e{\xx}$ can be viewed as a generalization of the sign vector. Observe also that $\e{\xx}=\proj_{\T_{\xx}}(\partial J(\xx))$, and thus $\e{\xx} \in \T_{\xx} \cap \Aff(\partial J(\xx))$. However, in general, $\e{\xx} \not\in \partial J(\xx)$.


We now provide a fundamental equivalent description of the subdifferential of $J$ at $\xx$ in terms of $\e{\xx}$, $\T_{\xx}$, $\S_{\xx}$ and the polar gauge $J^\circ$.
\begin{theorem}\label{thm:decomp}
Let $J$ satisfy \ref{assump:J}. Let $\xx \in \RR^p$ and $\f{\xx} \in \ri(\partial J(\xx))$.
\begin{enumerate}[label=(\roman*)]
\item The subdifferential of $J$ at $\xx$ reads
  \begin{align*}
    \partial J(\xx) &= \Aff(\partial J(\xx)) \cap \calC^\circ \\
    &=
    \enscond{\bseta \in \RR^n}
    {
      \bseta_{\T_{\xx}} = \e{\xx}
      \qandq
      \inf_{\tau \geq 0}\max\pa{J^\circ\pa{\tau\e{\xx} + \bseta_{\S_{\xx}} + (\tau-1)\proj_{\S_{\xx}}\f{\xx}},\tau} \leq 1
    } .
  \end{align*}
\item For any $\bsom \in \RR^p$, $\exists \bseta \in \partial J(\xx)$ such that
\[
J(\bsom_{\S_{\xx}}) = \dotp{\bseta_{\S_{\xx}}}{\bsom_{\S_{\xx}}} .
\]
\end{enumerate}
\end{theorem}

\begin{proof}
\begin{enumerate}[label=(\roman*)]
\item This follows by piecing together \cite[Theorem~1, Proposition~4 and Proposition~5(iii)]{vaiterimaiai13}.
\item From \cite[Proposition~5(iv)]{vaiterimaiai13}, we have
\[
\sigma_{\partial J(\xx) - \f{\xx}}(\bsom) = J(\bsom_{\S_{\xx}}) - \dotp{\proj_{\S_{\xx}}\f{\xx}}{\bsom_{\S_{\xx}}} .
\]
Thus there exists a supporting point $\bsv \in \partial J(\xx) - \f{\xx} \subset \S_{\xx}$ with normal vector $\bsom$ \cite[Corollary~7.6(iii)]{bauschke2011convex}, i.e.
\[
\sigma_{\partial J(\xx) - \f{\xx}}(\bsom) = \dotp{\bsv}{\bsom_{\S_{\xx}}} .
\]
Taking $\bseta=\bsv+\f{\xx}$ concludes the proof.
\end{enumerate}
\end{proof}

\begin{remark}
The coercivity assumption in \ref{assump:J} is not needed for Theorem~\ref{thm:decomp} to hold.
\end{remark}

The decomposability of described in Theorem~\ref{thm:decomp} depends on the particular choice of the $\f{\xx} \in \ri(\partial J(\xx))$. An interesting situation is encountered when $\e{\xx} \in \ri(J(\xx))$, so that one can choose $\f{\xx}=\e{\xx}$. Strong gauges, see \cite[Definition~6]{vaiterimaiai13}, are precisely a class of gauges for which this situation occurs, and in this case, Theorem~\ref{thm:decomp} has the simpler form
\begin{equation}\label{eq:decompstrong}
\partial J(\xx) = \Aff(\partial J(\xx)) \cap \calC^\circ =
\enscond{\bseta \in \RR^n}
{
  \bseta_{\T_{\xx}} = \e{\xx}
  \qandq
  J^\circ(\bseta_{\S_{\xx}}) \leq 1
} .
\end{equation}

The Lasso, group Lasso and nuclear norms are typical examples of (symmetric) strong gauges. However, group-analysis sparsity penalties such as the fused Lasso or the $\ell_\infty$-penalty are not strong gauges, though they obviously satisfy \ref{assump:J}. See the next section for a detailed discussion.


\subsection{Examples}\label{subsec:decompexamples}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Lasso}

\subsubsection{Group Lasso}

\subsubsection{Group-Analysis (group) Lasso, even with overlapping groups}

\subsubsection{Anti-sparsity}

\subsubsection{Nuclear norm}



==> sections/implementation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Numerical experiments} \label{sec:ne}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> sections/soiapplications_old.tex <==
\section{Applications}\label{subsec:SOIapp}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we exemplify our oracle inequalities for the penalties described in Section~\ref{subsec:decompexamp}.

\subsection{Lasso}
To lighten the notation, let $I_{\xx}=\supp(\xx)$. From \eqref{eq:exlasso}, it is easy to see that
\[
\normOP{\proj_{\T_{\xx}}}{2}{1} = \sqrt{|I_{\xx}|} \qandq J^\circ(\e{\xx}) = \anorm{\sign(\xx_{I_\xx})}{\infty} \leq 1 ,
\]
where last bound holds as an equality whenever $\xx \neq 0$. We now bound the probability of the event $\ens{\lambda \geq \tau \norm{\XX^\top\bsxi}{\infty}/n}$ when the noise is subgaussian, which entails the following corollary.

\begin{corollary}\label{cor:SOIlasso}
Let the data generated by \eqref{eq:obs} with noise $\bsxi$ whose entries are $n$ {\it iid} subgaussian centered random variables with parameter $\sigma$. Assume that $\XX$ is such that $\max_i\anorm{\XX_i}{2}\leq\sqrt{n}$. Consider the estimators $\thewa$ and $\thvar$, where $J$ is the Lasso penalty \eqref{eq:Jlasso} and $F$ satisfies Assumptions~\ref{assump:F}-\ref{assump:Fmom}. Let $0 < \epsilon < \nu$. Suppose that $\lambda \geq \tau\sigma\sqrt{\frac{2\log(2p/\delta)}{n}}$, for some $\tau > 1$ and $\delta \in ]0,1[$. Then, with probability at least $1-\delta$, the following holds
\begin{align}\label{eq:SOIEWAlasso}
R_n\bpa{\thewa,\xx_0} \leq & \inf_{\substack{I \subset \ens{1,\ldots,p} \\ \xx:~\supp(\xx)=I}} \pa{R_n\bpa{\xx,\xx_0} + \tfrac{\lambda^2\pa{\tau+1}^2|I|}{2\tau^2(\nu-\epsilon)\cfac{\Span\ens{\bs a_i}_{i \in I}}{\tfrac{\tau+1}{\tau-1}}^2}} \nonumber\\
			   & + p\beta + \frac{1}{2n\epsilon}\norm{\pa{\Id - \nabla\varphi}(\XX\xx_0)}{2}^2 ,
\end{align}
and
\begin{align}\label{eq:SOIPENlasso}
R_n\bpa{\thvar,\xx_0} \leq & \inf_{\substack{I \subset \ens{1,\ldots,p} \\ \xx:~\supp(\xx)=I}} \pa{R_n\bpa{\xx,\xx_0} + \tfrac{\lambda^2\pa{\tau+1}^2|I|}{2\tau^2(\nu-\epsilon)\cfac{\Span\ens{\bs a_i}_{i \in I}}{\tfrac{\tau+1}{\tau-1}}^2}} \nonumber\\
			   & + \frac{1}{2n\epsilon}\norm{\pa{\Id - \nabla\varphi}(\XX\xx_0)}{2}^2 .
\end{align}
\end{corollary}

When $\varphi$ is quadratic, the oracle inequality \eqref{eq:SOIPENlasso} recovers \cite[Theorem~1]{dalalyan16} in the exactly sparse case. \eqref{eq:SOIPENlasso} also coincides in this case with the oracle inequaliy in \cite[Theorem~4]{sunzhang} (see also \cite[Theorem2]{dalalyan17}). The first term in the remainder grows as $\tfrac{|I|\log(p)}{n}$ which is the classical scaling under the individual sparsity scenario.

\begin{proof}
By the union bound, we have
\begin{eqnarray*}
\PP{\norm{\XX^\top\bsxi}{\infty}>\epsilon}\le \PP{\bigcup_{i=1}^p |\dotp{\XX_i}{\bsxi}|>\epsilon} \leq \sum_{i=1}^p \PP{|\dotp{\XX_i}{\bsxi}|>\epsilon}\le p \max_{i\in \ens{1,\ldots,p}}\PP{|\dotp{\XX_i}{\bsxi}|>\epsilon} .
\end{eqnarray*}
Since $\bsxi_1,\ldots,\bsxi_n$ are $n$ {\it iid} subgaussian centered random variables with parameter $\sigma^2$, for any $i \in \{1,\ldots,p\}$, $\dotp{\XX_i}{\bsxi}$ is a sum of $n$ random variables {\it iid} subgaussian centered random variables with parameter $\sigma^2 \XX^2_{i,j}$. Owing to the Hoeffding bound\footnote{Note that the Hoeffding bound is originally stated for almost surely bounded random variables. However, one can easily check that the same bound applies more generally to subgaussian variables thanks to Cram\'er's theorem.}~\cite{Hoeffding63}, we obtain
\[
\PP{|\dotp{\XX_i}{\bsxi}|>\epsilon} \le 2 \exp\bpa{- \epsilon^2 / \bpa{2\sigma^2 \anorm{\XX_i}{2}^2}}.
\]
Taking $\epsilon=\lambda n/\tau$, we conclude.
\end{proof}

\subsection{Group Lasso}
Recall the notations in Section~\ref{subsec:decompglasso}, and denote $I_{\xx}=\bsupp(\xx)$ the number of active blocks in $\xx$. From \eqref{eq:exglasso}, we have
\[
\normOP{\proj_{\T_{\xx}}}{2}{J} = \sqrt{|I_{\xx}|} \qandq J^\circ(\e{\xx}) = \anorm{\e{\xx}}{\infty,2} \leq 1 ,
\]
where the last bound holds as an equality whenever $\xx \neq 0$.

When the noise is {\it iid} Gaussian, we get the following oracle inequalities.

\begin{corollary}\label{cor:SOIglasso}
Let the data generated by \eqref{eq:obs} with noise $\bsxi$ whose entries are $n$ {\it iid} $\calN(0,\sigma^2)$. Consider the estimators $\thewa$ and $\thvar$, where $F$ satisfies Assumptions~\ref{assump:F}-\ref{assump:Fmom}, and $J$ is the group Lasso \eqref{eq:Jglasso} with $L$ non-overlapping blocks of equal size $K$. Assume that $\XX$ is such that $\max_i\normOP{\XX_{b_i}^\top\XX_{b_i}}{2}{2}\leq n$. Let $0 < \epsilon < \nu$. Suppose that $\lambda \geq \tau\sigma\sqrt{\frac{K+2\pa{2\delta\log(L)+\sqrt{K\delta\log(L)}}}{n}}$, for some $\tau > 1$ and $\delta > 1$. Then, with probability at least $1-2L^{1-\delta}$, the following holds
\begin{align}\label{eq:SOIEWAglasso}
R_n\bpa{\thewa,\xx_0} \leq & \inf_{\substack{I \subset \ens{1,\ldots,L} \\ \xx:~\bsupp(\xx)=I}} \pa{R_n\bpa{\xx,\xx_0} + \tfrac{\lambda^2\pa{\tau+1}^2|I|}{2\tau^2(\nu-\epsilon)\cfac{\Span\ens{a_j}_{j \in b_i, i \in I}}{\tfrac{\tau+1}{\tau-1}}^2}} \nonumber\\
			   & + p\beta + \frac{1}{2n\epsilon}\norm{\pa{\Id - \nabla\varphi}(\XX\xx_0)}{2}^2 ,
\end{align}
and
\begin{align}\label{eq:SOIPENglasso}
R_n\bpa{\thvar,\xx_0} \leq & \inf_{\substack{I \subset \ens{1,\ldots,L} \\ \xx:~\bsupp(\xx)=I}} \pa{R_n\bpa{\xx,\xx_0} + \tfrac{\lambda^2\pa{\tau+1}^2|I|}{2\tau^2(\nu-\epsilon)\cfac{\Span\ens{a_j}_{j \in b_i, i \in I}}{\tfrac{\tau+1}{\tau-1}}^2}} \nonumber\\
			   & + \frac{1}{2n\epsilon}\norm{\pa{\Id - \nabla\varphi}(\XX\xx_0)}{2}^2 .
\end{align}
\end{corollary}

The first remainder term is on the order $\frac{|I|\pa{\sqrt{K}+\sqrt{2\log(L)}}^2}{n}$, which is similar to the scaling that has been provided in the literature for EWA with other group sparsity priors~\cite{rigo12,luu16}. Similar rates were given for $\thvar$ with group Lasso in \cite{negahban2010unified,lounici11,vandegeer14}.

\begin{proof}
The proof is essentially an adaptation of \cite[Lemma~3.1]{lounici11}, where we also used that for all $i=1,\ldots,L$,
\[
n^{-1}\tr\bpa{\XX_{b_i}^\top\XX_{b_i}} \leq K n^{-1} \anormOP{\XX_{b_i}^\top\XX_{b_i}}{2}{2} \leq K .
\]
\end{proof}

\subsection{Analysis (group) Lasso}
We now turn to the prior penalty \eqref{eq:Janaglasso}. Recall the notations in Section~\ref{subsec:decompanaglasso}, and remind $\Lambda_{\xx}=\bigcup_{i \in \bsupp(\bsD^\top\xx)} b_i$. We assume that $\bsD$ is a frame of $\RR^p$, hence surjective, meaning that there exist $c, d > 0$ such that for any $\bsom \in \RR^p$
\[
d \anorm{\bsom}{2}^2 \leq \norm{\bsD^\top \bsom}{2}^2 \leq c \anorm{\bsom}{2}^2 .
\]
This together with \eqref{eq:exanaglasso}-\eqref{eq:exanaglassoJo} and Cauchy-Schwarz inequality entail
\begin{align*}
\normOP{\proj_{\T_{\xx}}}{2}{J} = \sup_{\anorm{\bsom_{\T_{\xx}}}{2} \leq 1} \norm{\bsD^\top \bsom_{\T_{\xx}}}{1,2}
				&\leq \sqrt{c}\sup_{\anorm{\bsD^\top\bsom_{\T_{\xx}}}{2} \leq 1} \norm{\bsD^\top \bsom_{\T_{\xx}}}{1,2} \\
				&= \sqrt{c}\sup_{\anorm{\bsD_{\Lambda_{\xx}}^\top\bsom_{\T_{\xx}}}{2} \leq 1} \norm{\bsD_{\Lambda_{\xx}}^\top \bsom_{\T_{\xx}}}{1,2} \\
				&= \sqrt{c}\sqrt{|\bsupp(\bsD^\top\xx)|} .
%				&= \sup_{\anorm{\proj_{\Span\ens{\bs a_i}_{i \in \Lambda_{\xx}}}\bsD^\top\bsom_{\T_{\xx}}}{2} \leq 1} \anorm{\proj_{\Span\ens{\bs a_i}_{i \in \Lambda_{\xx}}}\bsD^\top \bsom_{\T_{\xx}}}{1,2} \\
%				&= \sup_{\lrcurly{\anorm{\proj_{\Span\ens{\bs a_i}_{i \in \Lambda_{\xx}}}\bsom}{2} \leq 1} \cap \Span\pa{(\bsD^\top)_{\T_{\xx}}}} \anorm{\proj_{\Span\ens{\bs a_i}_{i \in \Lambda_{\xx}}}\bsom}{1,2} \\
%				&\leq \anormOP{\proj_{\Span\ens{\bs a_i}_{i \in \Lambda_{\xx}}}}{2}{\anorm{\cdot}{1,2}} = \sqrt{|I_{\bsD^\top\xx}|} .
\end{align*}
However, from \eqref{eq:exanaglasso}, we do not have in general $\anorm{\bsD^+\proj_{\Ker(\bsD^\top_{\Lambda^c_{\xx}})}\bsD\e{\bsD^\top \xx}^{\anorm{}{1,2}}}{\infty,2} \leq 1$.

With arguments analogue to those for proving Corollary~\ref{cor:SOIglasso}, we arrive at the following oracle inequalities.

\begin{corollary}\label{cor:SOIanaglasso}
Let the data generated by \eqref{eq:obs} with noise $\bsxi$ whose entries are $n$ {\it iid} $\calN(0,\sigma^2)$. Consider the estimators $\thewa$ and $\thvar$, where $F$ satisfies Assumptions~\ref{assump:F}-\ref{assump:Fmom}, and $J$ is the analysis group Lasso \eqref{eq:Janaglasso} with $L$ blocks of equal size $K$. Assume that $\bsD$ is a frame, and $\XX$ is such that $\max_i\normOP{\bsD_{b_i}^\top\XX^\top\XX\bsD_{b_i}}{2}{2}\leq n$. Let $0 < \epsilon < \nu$. Suppose that $\lambda \geq \tau\sigma\sqrt{\frac{K+2\pa{2\delta\log(L)+\sqrt{K\delta\log(L)}}}{n}}$, for some $\tau > 1$ and $\delta > 1$. Then, with probability at least $1-2L^{1-\delta}$, the following holds
\begin{align}\label{eq:SOIEWAanaglasso}
R_n\bpa{\thewa,\xx_0} \leq & \inf_{\substack{I \subset \ens{1,\ldots,L} \\ \xx:~\bsupp(\bsD^\top\xx)=I}} \pa{R_n\bpa{\xx,\xx_0} + \tfrac{c\lambda^2\bpa{\tau\norm{\bsD^+\proj_{\Ker(\bsD^\top_{\Lambda^c_{\xx}})}\bsD\e{\bsD^\top \xx}^{\anorm{}{1,2}}}{\infty,2}+1}^2|I|}{2\tau^2(\nu-\epsilon)\acfac{\Ker(\bsD^\top_{\Lambda^c_{\xx}})}{\tfrac{\tau\norm{\bsD^+\proj_{\Ker(\bsD^\top_{\Lambda^c_{\xx}})}\bsD\e{\bsD^\top \xx}^{\anorm{}{1,2}}}{\infty,2}+1}{\tau-1}}^2}} \nonumber\\
			   & + p\beta + \frac{1}{2n\epsilon}\norm{\pa{\Id - \nabla\varphi}(\XX\xx_0)}{2}^2 ,
\end{align}
and
\begin{align}\label{eq:SOIPENanaglasso}
R_n\bpa{\thvar,\xx_0} \leq & \inf_{\substack{I \subset \ens{1,\ldots,L} \\ \xx:~\bsupp(\bsD^\top\xx)=I}} \pa{R_n\bpa{\xx,\xx_0} + \tfrac{c\lambda^2\bpa{\tau\norm{\bsD^+\proj_{\Ker(\bsD^\top_{\Lambda^c_{\xx}})}\bsD\e{\bsD^\top \xx}^{\anorm{}{1,2}}}{\infty,2}+1}^2|I|}{2\tau^2(\nu-\epsilon)\acfac{\Ker(\bsD^\top_{\Lambda^c_{\xx}})}{\tfrac{\tau\norm{\bsD^+\proj_{\Ker(\bsD^\top_{\Lambda^c_{\xx}})}\bsD\e{\bsD^\top \xx}^{\anorm{}{1,2}}}{\infty,2}+1}{\tau-1}}^2}} \nonumber\\
			   & + \frac{1}{2n\epsilon}\norm{\pa{\Id - \nabla\varphi}(\XX\xx_0)}{2}^2 .
\end{align}
\end{corollary}

To the best of our knowledge, this result is new to the literature. The scaling of the remainder term is the same as in \cite[Remark~6.2]{luu16} and \cite{rigo12} with analysis sparsity priors different from ours (the authors in the latter also assume that $\bsD$ is invertible).

\subsection{Anti-sparsity}
From Section~\ref{subsec:decomplinf}, recall the saturation support $\Isat_{\xx}$ of $\xx$. From \eqref{eq:exlinf}, we get
\[
\normOP{\proj_{\T_{\xx}}}{2}{\infty} = 1 \qandq J^\circ(\e{\xx}) = \norm{\sign(\xx_{\Isat_{\xx}})}{1}/|\Isat_{\xx}| \leq 1 ,
\]
with equality whenever $\xx \neq 0$.

Assuming that the noise is {\it iid} zero-mean Gaussian, we get the following oracle inequalities.

\begin{corollary}\label{cor:SOIlinf}
Let the data generated by \eqref{eq:obs} with noise $\bsxi$ whose entries are $n$ {\it iid} $\calN(0,\sigma^2)$. Assume that $\XX$ is such that $\max_{i,j}|\XX_{i,j}|\leq 1/\sqrt{n}$. Consider the estimators $\thewa$ and $\thvar$, where $F$ satisfies Assumptions~\ref{assump:F}-\ref{assump:Fmom}, and $J$ is the anti-sparsity penalty \eqref{eq:Jlinf}. Let $0 < \epsilon < \nu$. Suppose that $\lambda \geq \sqrt{\tfrac{2}{\pi}}\tau(1+\delta)\sigma p/n$, for some $\tau > 1$ and $\delta > 0$. Then, with probability at least $1-e^{-\tfrac{\delta^2}{\pi}}$, the following holds
\begin{align}\label{eq:SOIEWAlinf}
R_n\bpa{\thewa,\xx_0} \leq & \inf_{\substack{I \subset \ens{1,\ldots,p} \\ \xx:~\Isat_{\xx}=I}} \pa{R_n\bpa{\xx,\xx_0} + \tfrac{\lambda^2\pa{\tau+1}^2}{2\tau^2(\nu-\epsilon)\cfac{\enscond{\bxx}{\bxx_{I} \in \RR \sign(\xx_{I})}}{\tfrac{\tau+1}{\tau-1}}^2}} \nonumber\\
			   & + p\beta + \frac{1}{2n\epsilon}\norm{\pa{\Id - \nabla\varphi}(\XX\xx_0)}{2}^2 ,
\end{align}
and
\begin{align}\label{eq:SOIPENlinf}
R_n\bpa{\thvar,\xx_0} \leq & \inf_{\substack{I \subset \ens{1,\ldots,p} \\ \xx:~\Isat_{\xx}=I}} \pa{R_n\bpa{\xx,\xx_0} + \tfrac{\lambda^2\pa{\tau+1}^2}{2\tau^2(\nu-\epsilon)\cfac{\enscond{\bxx}{\bxx_{I} \in \RR \sign(\xx_{I})}}{\tfrac{\tau+1}{\tau-1}}^2}} \nonumber\\
			   & + \frac{1}{2n\epsilon}\norm{\pa{\Id - \nabla\varphi}(\XX\xx_0)}{2}^2 .
\end{align}
\end{corollary}

We are not aware of any result of this kind in the literature. The first remainder term scales as $\pa{\tfrac{p}{n}}^2$. The bound imposed on $\XX$ is similar to what is generally assumed in the vector quantization literature~\cite{lyubarskii2010uncertainty,studer12signal}.

\begin{proof}
The function $\bsxi \mapsto \anorm{\XX^\top\bsxi}{1}$ is Lipschitz continuous with Lipschitz constant $\sum_{i=1}^p\anorm{\XX_i}{2}$. Moreover, $\EE{}{\norm{\XX^\top\bsxi}{1}}=\sqrt{\tfrac{2}{\pi}}\sigma\sum_{i=1}^p\anorm{\XX_i}{2} \leq \sqrt{\tfrac{2}{\pi}}\sigma p$. Invoking Proposition~\ref{prop:SOIprobgw} concludes the proof.
%$\epsilon=\lambda n/\tau - \sqrt{\tfrac{2}{\pi}}\sigma\sum_{i=1}^p\anorm{\XX_i}{2} \geq \delta\sqrt{\tfrac{2}{\pi}}\sigma \sum_{i=1}^p\anorm{\XX_i}{2}$, it follows from the Gaussian concentration of Lipschitz functions~\cite{ledouxbook} that
%\begin{align*}
%\PP{\norm{\XX^\top\bsxi}{1} \geq \lambda n/\tau} 
%	&=\PP{\norm{\XX^\top\bsxi}{1} - \EE{}{\norm{\XX^\top\bsxi}{1}} > \epsilon} \\
%	&\leq \exp\pa{-\frac{\bpa{\lambda n/\tau - \sqrt{\tfrac{2}{\pi}}\sigma\sum_{i=1}^p\anorm{\XX_i}{2}}^2}{2\sigma^2\bpa{\sum_{i=1}^p\anorm{\XX_i}{2}}^2}} \\
%	&\leq \exp\pa{-\frac{\delta^2}{\pi}} .
%\end{align*}
\end{proof}

\subsection{Nuclear norm}
We now turn to the nuclear norm case. Recall the notations of Section~\ref{subsec:decompnuc}. For matrices $\xx \in \RR^{p_1 \times p_2}$, a measurement map $\XX$ takes the form of a linear operator whose $i$th component is given by the Frobenius scalar product
\[
\XX(\xx)_i = \tr((\XX^i)^\top \xx) = \dotp{\XX^i}{\xx}_{\mathrm{F}} ,
\]
where $\XX^i$ is a matrix in $\RR^{p_1 \times p_2}$. We denote $\anorm{\cdot}{F}$ the associated norm. From \eqref{eq:exnuc}, it is immediate to see that whenever $\xx \neq 0$,
\[
J^\circ(\e{\xx}) = \anormOP{\bs U \bs V^\top}{2}{2} = 1.
\]
Moreover, since 
\[
\anorm{\xx}{*} = \anorm{\uplambda(\xx)}{1} \leq \sqrt{r}\anorm{\uplambda(\xx)}{2} = \sqrt{r}\anorm{\xx}{\mathrm{F}} ,
\]
we deduce that
\[
\normOP{\proj_{\T_{\xx}}}{\mathrm{F}}{*} = \sqrt{r} .
%= \inf_{\bsom \in \T_{\xx}} \sqrt{\rank(\bsom)} \leq \sqrt{\rank(\xx)} = \sqrt{r} ,
\]
%since $\xx \in \T_{\xx}$ (see Section~\ref{subsec:decomp}). 
For standard Gaussian noise $\bsxi$, we need to bound 
\[
\normOP{\XX^*(\bsxi)}{2}{2}=\normOP{\sum_{i=1}^n\XX_i\bsxi_i}{2}{2} ,
\] 
which is the operator norm of a random series with matrix coefficients. Thus arguing as in \cite[Lemma~6]{dalalyan16} (which relies on \cite[Theorem~4.1.1]{tropp15}, we get the following oracle inequalities for the nuclear norm. Define 
\[
v(\XX) = \max\pa{\normOP{\sum_{i=1}^n \XX^i(\XX^i)^\top}{2}{2},\normOP{\sum_{i=1}^n (\XX^i)^\top\XX^i}{2}{2}} .
\]

\begin{corollary}\label{cor:SOInuc}
Let the data generated by \eqref{eq:obs} with a linear operator $\XX: \RR^{p_1 \times p_2} \to \RR^n$, with noise $\bsxi$ whose entries are $n$ {\it iid} $\calN(0,\sigma^2)$. Assume that $v(\XX) \leq n$. Consider the estimators $\thewa$ and $\thvar$, where $F$ satisfies Assumptions~\ref{assump:F}-\ref{assump:Fmom}, and $J$ is the nuclear norm \eqref{eq:Jlinf}. Let $0 < \epsilon < \nu$. Suppose that $\lambda \geq \tau\sigma\sqrt{\frac{2\log((p_1+p_2)/\delta)}{n}}$, for some $\tau > 1$ and $\delta > 0$. Then, with probability at least $1-\delta$, the following holds
\begin{align}\label{eq:SOIEWAnuc}
R_n\bpa{\thewa,\xx_0} \leq & \inf_{\substack{r \in \ens{1,\ldots,\min(p_1,p_2)} \\ \xx:~\rank{\xx}=r}} \pa{R_n\bpa{\xx,\xx_0} + \tfrac{\lambda^2\pa{\tau+1}^2 r}{2\tau^2(\nu-\epsilon)\cfac{\T_{\xx}}{\tfrac{\tau+1}{\tau-1}}^2}} \nonumber\\
			   & + p_1p_2\beta + \frac{1}{2n\epsilon}\norm{\pa{\Id - \nabla\varphi}(\XX\xx_0)}{2}^2 ,
\end{align}
and
\begin{align}\label{eq:SOIPENnuc}
R_n\bpa{\thvar,\xx_0} \leq & \inf_{\substack{r \in \ens{1,\ldots,\min(p_1,p_2)} \\ \xx:~\rank{\xx}=r}} \pa{R_n\bpa{\xx,\xx_0} + \tfrac{\lambda^2\pa{\tau+1}^2 r}{2\tau^2(\nu-\epsilon)\cfac{\T_{\xx}}{\tfrac{\tau+1}{\tau-1}}^2}} \nonumber\\
			   & + \frac{1}{2n\epsilon}\norm{\pa{\Id - \nabla\varphi}(\XX\xx_0)}{2}^2 .
\end{align}
\end{corollary}

The set over which the infimum is taken just reminds us that the nuclear norm is partly smooth (see above) relative to the constant rank manifold (which is a Riemannian submanifold of $\RR^{p_1 \times p_2}$)~\citep[Theorem~3.19]{daniilidis2013orthogonal}. The first remainder term now scales as $\frac{r\log(p_1+p_2)}{n}$ and we recover the same rate as in \cite[Theorem~3]{dalalyan16} for $\thewa$ and in \cite[Theorem~2]{koltchinskii11} for $\thvar$.

